Methods for Pruning Deep Neural Networks

This paper presents a survey of methods for pruning deep neural networks. It begins by categorising over 150 studies based on the underlying approach used and then focuses on three categories: methods that use magnitude based pruning, methods that utilise clustering to identify redundancy, and methods that use sensitivity analysis to assess the effect of pruning. Some of the key influencing studies within these categories are presented to highlight the underlying approaches and results achieved. Most studies present results which are distributed in the literature as new architectures, algorithms and data sets have developed with time, making comparison across different studied difficult. The paper therefore provides a resource for the community that can be used to quickly compare the results from many different methods on a variety of data sets, and a range of architectures, including AlexNet, ResNet, DenseNet and VGG. The resource is illustrated by comparing the results published for pruning AlexNet and ResNet50 on ImageNet and ResNet56 and VGG16 on the CIFAR10 data to reveal which pruning methods work well in terms of retaining accuracy whilst achieving good compression rates. The paper concludes by identifying some promising directions for future research.

==> Pruning_Survey_Version 2/appendices.tex <==

%\documentclass[smallextended]{svjour3} 
%\documentclass[smallcondensed]{svjour3}     % onecolumn (ditto)
%\documentclass[smallextended]{svjour3}       % onecolumn (second format)
%\documentclass[twocolumn]{svjour3}          % twocolumn
%\usepackage{natbib}
%\usepackage[numbers]{natbib}
% \bibliographystyle{unsrt}
%\usepackage{amsfonts}
%\usepackage{amstext}
%\usepackage{amsmath}
%
%\smartqed  % flush right qed marks, e.g. at end of proof
%
%\usepackage{graphicx}
%
%\usepackage{mathptmx}      % use Times fonts if available on your TeX system
%
% insert here the call for the packages your document requires
%\usepackage{latexsym}
% etc.
%
% please place your own definitions here and don't use \def but
% \newcommand{}{}
%
\newcommand{\rot}{\rotatebox{90}}

%\newcommand{\R}{\mathbb{R}}
% Insert the name of "your journal" with
% \journalname{myjournal}
%
%\begin{document}
%	\title{Methods for Pruning Deep Neural Networks}
%	\author{Sunil Vadera \and Salem Ameen}
%	\institute{S.Vadera, University of Salford, \email{S.Vadera@salford.ac.uk}
%		\and 
%		S.Ameen, University of Salford, \email{S.Ameen@salford.ac.uk}
%	}
%	\date{Received: date / Accepted: date}
%	\maketitle
%\clearpage
\section*{\bf Appendix A: Categorisation of Studies on Pruning}
%\begin{table}[h]
\begin{small}
	\begin{tabular}{|l|l|}\hline \hline
		\multicolumn{2}{l}{\bf Magnitude based pruning methods} \\ \hline
		1988-91& \cite{Kruschke1988, Hanson1989,Weigend1990,Weigend1991} \\ \hline
		2011 & \cite{Graves2011} \\ \hline
		2015 & \cite{Han2015a,Polyak2015}\\ \hline
		2016 &\cite{Guo2016,Hu2016,Wen2016} \\ \hline
		2017 & \cite{Aghasi2017,He2017,Li2017,Liu2017,Luo2017a,Luo2017} \\
		     & \cite{Wang2017,Zhu2017} \\ \hline
		2018 &	\cite{Chen2018,He2018,Huang2018,Lee2018a}\\
		     & \cite{Li2018,Liu2018d,Luo2018,Qin2018}\\
		     & \cite{Yazdani2018,Ye2018, Yu2018, Zhang2018a, Zhou2018} \\ \hline
		2019 &	\cite{Ding2019,Ding2019c,Dettmers2019, Frankle2019,Frankle2019a}   \\ 
			&  \cite{Gui2019, He2019, Helwegen2019, Hou2019, Lee2019, Li2019} \\
			& \cite{Liu2019, Liu2019a, Mittal2019, Morcos2019, Song2019, Xu2019}\\
			& \cite{Yu2019, Zhao2019a,Zhou2019,Zhu2019} \\ \hline
		2020 &	\cite{Hubens2020,Kim2020, Li2020, Lin2020, Lin2020b, Niu2020} \\ \hline
		\multicolumn{2}{l}{\bf Similarity and clustering methods  } \\ \hline
	2017 &	\cite{RoyChowdhury2017}\\ \hline
	2018 &	\cite{Dubey2018, Son2018}\\ \hline
	2019 &	\cite{Ayinde2019, Ding2019b, Li2019b,Li2019sv} \\	\hline 
	2021 & \cite{Lin2021} \\ \hline
	\multicolumn{2}{l}{\bf Sensitivity analysis methods}\\ \hline 
	1988 &	\cite{Mozer1988}\\ \hline
	1990 &	\cite{LeCun1990}\\	\hline
	1992-1993 &	\cite{Hassibi1992,Hassibi1993,Hassibi1993a}\\ \hline
	2006-2009 &  \cite{Xu2006, Endisch2007,Endisch2009} \\ \hline
	2016 &	\cite{Cohen2016,Grosse2016,Molchanov2016a} \\	\hline
	2017 &	 \cite{Ameen2017,Anwar2017, Dong2017}  \\
		 & \cite{Guo2017, Neklyudov2017} \\ \hline
	2018 & \cite{Lin2018,Bao2018,Carreira-Perpinan2018,Jiang2018} \\ 
		 & \cite{Huang2018a,Huynh2018,Zhuang2018} \\ \hline
	2019 &	\cite{Chen2019a,Deng2019,Jin2019,Lee2018} \\
		 &  \cite{Li2019c,Molchanov2019,Peng2019,Qin2019, Wang2019, Xiao2019}	\\ \hline
	2020 & \cite{Ameen2020} \\ \hline
	\multicolumn{2}{l}{\bf Knowledge distillation methods}\\ \hline
	2006  &	\cite{Bucilua2006}  \\	\hline
	2014-2017 &	\cite{Romero2014,Hinton2015,GregorUrban2017} \\	\hline
	2019 &	\cite{Bao2019, Lemaire2019, Zhang2019a, Dong2019}  \\ \hline
	2020 & \cite{kundu2020} \\ \hline
	2021 & \cite{Kaliamoorthi2021} \\ \hline
	\multicolumn{2}{l}{\bf Methods based on rank and reconstruction} \\\hline
	2013-2016 &	\cite{Sainath2013,Jaderberg2014,Lebedev2015,Zhang2016} \\	\hline
	2018 &	\cite{Lin2018a} \\	\hline
	2020 &	\cite{Lin2020c}\\	\hline
	\multicolumn{2}{l}{\bf Quantization methods}\\\hline
	2011 & \cite{Vanhoucke2011}  \\ \hline
	2014-17 &	\cite{Denton2014,Gong2014,Chen2015,Hubara2016,Rastegari2016,Zhou2017a} \\ \hline
	2018 &	\cite{Jacob2018,Krishnamoorthi2018,Liu2018a,Tung2018} \\ \hline
	2019 &  \cite{Banner2019,Chen2019, Jung2019,Zhao2019} \\  \hline
	2020 &  \cite{Wang2020} \\ \hline
	2021 &  \cite{Stock2021} \\ \hline
	\multicolumn{2}{l}{\bf Architectural design methods} \\\hline
	2017 &	\cite{Baker2017, Howard2017, Lin2017, Zoph2017} \\ \hline
	2018 & 	\cite{Gordon2018, He2018a,Hsu2018,liu2018progressive,Pham2018,Zhong2018}\\ \hline
	2019 & \cite{Dai2019,Esteban2019, Liu2019metapruning,Tan2019, Zhang2019b} \\\hline
	2020 & \cite{Elsen2020,Evci2020, Lin2020a} \\	\hline
	\multicolumn{2}{l}{\bf Hybrid Methods}\\ \hline
	2016 &	\cite{Chung2016, Han2016b} \\\hline
	2018-2019 &	\cite{Goetschalckx2018,Gadosey2019} \\ \hline
	\multicolumn{2}{l}{\bf Survey Papers}\\ \hline
	1993 &	\cite{Reed1993} \\ \hline
	2018-2021 &	\cite{Cheng2018a, Cheng2018, Lebedev2018,Elsken2019,Menghani2021} \\ \hline \hline
\end{tabular}
%\caption{Categorisation of studies on pruning neural networks}
\end{small}
%\end{table}

\section*{Appendix B: Summary of Data Sets used in Comparing Pruning Methods}

%\begin{tabular}{|l|l|} \\ \hline
%Data set &	Brief Description  \\ \hline
\begin{description}
	
\item[MNIST~\citep{LeCun1998a}:]
The MNIST (Modified National Institute of Standards and Technology) data set consists of handwritten 28x28 images of digits.  It has 60,000 examples of training data and 10,000 examples for the test set.
\item[PASCAL VOC~\citep{Everingham2015}:] 
The PASCAL VOC data sets have formed the basis of an annual competitions from 2005 to 2012.  The VOC 2007 data annotates objects in 20 classes and consists of 9,963 images and 24,640 annotated objects.  The VOC 2012 data, which consists of 11530 images, are annotated with 27450 regions of interest and 6929 segmentations. 
\item[CamVid~\citep{Brostow2009}:]
CamVid (Cambridge-driving Labelled Video Database) is a data set with videos captured from an automobile. In total over 10mins of video is provided together with over 700 images from the videos that have been labelled.  Each pixel of an image is labelled to indicate if it is part of an objects in one of 32 semantic classes.  
\item[Oxford-Flowers~\citep{Nilsback2008}:]
The Oxford-Flowers data consists of 102 classes of common flowers in the UK.  It provides 2040 training images and 6129 images for testing.
\item[LFW ~\cite{Huang2008}:] The LFW (Labelled Faces in the Wild) is one of the largest and widely used data sets to evaluate face recognition algorithms.  It includes 250x250 pixel images of over 5.7K individuals, with over 13K images in total.
\item[CIFAR-10 \&100 ~\citep{Krizhevsky2009}:]
The CIFAR-10 (Canadian Institute for Advanced Research) data set is a collection of 32x32 colour images in 10 different classes. The data set splits into two sets: 50,000 images for training and 10,000 for testing. CIFAR-100 is similar to CIFAR-10 but has 100 classes, where each class has 500 training images and 100 test images.
\item[ImageNet~\citep{Deng2009}:]    
ImageNet contains millions of images organized using the WordNet hierarchy. It has over 14M images classified in over 21K groups and has provided the data sets for the ImageNet Large Scale Visual Recognition Challenges (ILSVRC) held since 2010.  It is one of the most widely used data sets in benchmarking deep learning models and methods for pruning. A smaller subset known as TinyImageNet is sometimes used and is also available (https://tiny-imagenet.herokuapp.com). It consists of 200 classes with 500 training, 50 validation and 50 testing images per class.  
\item[SVHN~\citep{Netzer2011}:]
The SVHN (Street View House Number) data set is a collection of 600K, 32x32 images of house numbers in Google Street View images. The data set provides 73,257 images for training and 26,032 for testing.
\item[UCSD-Birds~\citep{Wah2011}:]
The UCSD-Birds data set provides 11788 images of birds, labelled as one of 200 different types of species.  The data is split into training and testing sets of 5994 and 5794 respectively.   
\item[Places365~\citep{Zhou2014}:]
Places365 is a data set with 8 million 200x200 pixel images of scenes labeled with one of 434 categories, such as bridge, kitchen, boxing ring, etc.  It provides 50 images per class for validation and the test set consist of 500 images per class. 
\item[CASIA-WebFace~\citep{YiDong2014}:]
Zhen et al. 2014
[170]
CASIA-WebFace is a data set that was created for evaluating face recognition systems.  It provides over 494K  images of over 10K individuals.  
\item[WMT’14 En2De:\citep{Bojar2014}:]
WMT’14 En2De is one of the benchmark language data sets provided for a task set for the Workshop on Statistical Machine Translation held in 2014.   This data set consists of 4.5M English-German pairs of sentences. 
\item[FashionMNIST~\citep{Xiao2017fashionmnist}:]
FashionMNIST is an alternative  to the MNIST data set with  28x28  images of fashion products classified  in 10 categories.  Like MNIST, there are 60,000 images for training and 10,000 images for testing, 
\end{description}



\section*{Appendix C: Summary of Notation}

\begin{itemize}
	
	\item In general, we use $X $ to denote input channels, $W$ to denote weights of filters and $Y$ to denote output channels. 
	\item $Y_{i}$ j  is used to denote the output feature map obtained by applying a filter  $W_{j,i}$  on input channels $X_{i}$ 
	\item $w_{i}$, $w_{j}$, $w_{j,i}$ are used to denote individual weights.
	\item $\beta$ is used to denote a binary mask where $\beta_{i} = 1$ indicates that a feature map or filter should be retained and $\beta=0$ indicates that it should be removed.
	\item $\mathcal{L}$ is used to  denotes a loss function
	\item $L_{0}, L_{1}, L_{2}$ denote norms, with $L_{0}$ counting non-zero values, $L_{1}$, being the sum of absolute. values, $L_{2}$ being the square root of the sum of squares (Euclidean distance). 
	\item $\|W\|_{n}$ will be used to indicate the use of a norm in an equation with the an equation, with the subscript n indicating the specific norm.
	\item $\|W\|_{F}$, known as the Frobenius norm is sometimes used to denote the application of the Euclidean distance to the elements of a matrix
	
\end{itemize}

\section*{Appendix D: Number of Reported Results for a given Architecture and Data Set}
\begin{small}
	
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|}   \hline
& \rot{CALTECH256} & \rot{CamVid} & \rot{CIFAR10} & \rot{CIFAR100} &\rot{CUB200-2011} &\rot{Flowers102} & \rot{ImageNet} &\rot{MNIST} &\rot{Pascal VOC} &\rot{SVHN} &\rot{\bf Total} \\ 
		{\bf Architecture} & & & & & & & & & & & \\ \hline
		AlexNet & & & & & & &22 & & & &22 \\ \hline
		DenseNet-100 & & &3 & & & & & & & &3 \\ \hline
		DenseNet-40 & & &3 &1 & & & & & &2 &3 \\ \hline
		FCN32 & & & & & & & & &1 & &1 \\ \hline
		LeNet-300 & & & & & & & &9 & & &9 \\ \hline
		LeNet5 & & & & & & & &23 & & &23 \\ \hline
		Res101 & & & & & & &6 & & & &6 \\ \hline
		Res110 & & &13 & & & & & & & &13 \\ \hline
		Res152 & & & & & & &3 & & & &3 \\ \hline
		Res164 & & &1 &1 & & & & & & &1 \\ \hline
		Res18 &1 & &4 & &1 &1 &3 & & & &8 \\ \hline
		Res20 & & &6 & & & & & & & &6 \\ \hline
		Res32 & & &17 &10 & & & & & & &17 \\ \hline
		Res34 & & & & & & &3 & & & &3 \\ \hline
		Res50 & & & & & & &26 & & & &26 \\ \hline
		Res56 & & &20 & & & &1 & & & &21 \\ \hline
		SegNet  &1 & & & & & & & & &1 &\\ \hline
		VGG16 &1 & &13 &1 &3 &1 &10 & & & &24 \\ \hline
		VGG19 & & &12 &12 &1 & & & & & &13 \\ \hline
		{\bf Total} &1 &1 &48 &13 &3 &1 &59 &28 &1 &2 &115 \\ \hline
\end{tabular}
\end{small}

\clearpage

% BibTeX users please use one of
%\bibliographystyle{spbasic}      % basic style, author-year citations
%\bibliographystyle{spmpsci}      % mathematics and physical sciences
%\bibliographystyle{spphys}       % APS-like style for physics
%\bibliographystyle{num}
%\bibliographystyle{unsrt}
%\bibliography{survey}   % name your BibTeX data base

%\end{document}
